Transients of platoons with asymmetric and different Laplacians

We consider an asymmetric control of platoons of identical vehicles with nearest-neighbor interaction. Recent results show that if the vehicle uses different asymmetries for position and velocity errors, the platoon has a short transient and low overshoots. In this paper we investigate the properties of vehicles with friction. To achieve consensus, an integral part is added to the controller, making the vehicle a third-order system. We show that the parameters can be chosen so that the platoon behaves as a wave equation with different wave velocities. Simulations suggest that our system has a better performance than other nearest-neighbor scenarios. Moreover, an optimization-based procedure is used to find the controller properties.

==> notation.tex <==
%% Notation commands
\newcommand{\pos}{y} %car's position 
\newcommand{\err}{\tilde{e}} %spacing error 
\newcommand{\inp}{r} %input of the car -acceleration
\newcommand{\totalInput}{u}
\newcommand{\relCoupling}{c}

\newcommand{\dreference}{d_{\mathrm{ref}}} %reference distance
\newcommand{\drefVect}{{d}}
\newcommand{\vel}{v}
\newcommand{\weightGain}{\mu}

%% ODE coefficients
\newcommand{\contNumCoef}{q}
\newcommand{\contDenCoef}{p}
\newcommand{\vehNumCoef}{b}
\newcommand{\vehDenCoef}{a}
\newcommand{\olnum}{\psi} %numarator of open loop
\newcommand{\olden}{\phi} %denominator of open loop


%% Transfer functions
\newcommand{\vehicleTf}{G}
\newcommand{\controllerTf}{R}
\newcommand{\systemOutput}{y}
\newcommand{\systemOutputVect}{{\systemOutput}}
\newcommand{\controlEffort}{u}
\newcommand{\controlEffortVect}{{\controlEffort}}
\newcommand{\relOutDif}{\tilde{\systemOutput}}
\newcommand{\relOutDifVect}{\mathbf{\relOutDif}}
\newcommand{\regError}{E}
\newcommand{\regErrorVect}{\mathbf{\regError}}
\newcommand{\openLoop}{M}
\newcommand{\openLoopGain}{\openLoop_{\min}}
\newcommand{\olNumMat}{N}
\newcommand{\outWeightMat}{W}

\newcommand{\contNumOrd}{w}
\newcommand{\contDenOrd}{v}
\newcommand{\vehNumOrd}{m}
\newcommand{\olOrd}{n}
\newcommand{\wn}{i}

%weights of asymmetric bidirectional control
\newcommand{\wf}{1}
\newcommand{\wb}{\epsilon}
\newcommand{\wbmax}{\wb_{\max}}


% Constants
\newcommand{\numVeh}{N}

% % Functions
\newcommand{\drefWn}{\dreference_\wn}

% assumption

%%% ------- matrices and vectors -----------------
% laplacian and its eigenpairs
\newcommand{\lapl}{{L}}
\newcommand{\lapllf}{\lapl_{lf}} % laplacian with two leaders
\newcommand{\lapll}{\lapl_l} %laplacian with one leader
\newcommand{\redLapl}{{\lapl_\mathrm{r}}}
\newcommand{\redLaplCO}{\hat{\lapl}}
\newcommand{\redLapllf}{\bar{\lapl}_{lf}}
\newcommand{\laplz}{\lapl_z} % Laplacian to obtain zeros of the system
\newcommand{\spatEig}{\lambda} %laplacian eigenvalues
\newcommand{\spatEigWn}{\lambda_\wn}
\newcommand{\spatEigMin}{\spatEig_{\min}}
\newcommand{\spatEigMax}{\spatEig_{\max}}
\newcommand{\eigVect}{v} %laplacian eigenvectors
\newcommand{\eigVectGen}{\bar{\eigVect}}
\newcommand{\eigVectWn}{\eigVect_{\wn}}
\newcommand{\spatFreqWn}{\theta_\wn} %spatial frequency
\newcommand{\charPolCoef}{\alpha}
%zeros
\newcommand{\spatEigZ}{\gamma}
%jordan form
\newcommand{\matJ}{{J}}
\newcommand{\matEigVect}{{V}}
%graph 
\newcommand{\graph}{\mathcal{G}}
\newcommand{\vertSet}{\mathcal{V}}
\newcommand{\edgeSet}{\mathcal{E}}
\newcommand{\contNode}{C}
\newcommand{\obsvNode}{O}
\newcommand{\distance}{d}
\newcommand{\distanceCO}{\distance_{CO}}
\newcommand{\weight}{w}
\newcommand{\weightCO}{\weight_{CO}}

%state vector and matrices
\newcommand{\stateVect}{{x}}
\newcommand{\stateVectMod}{{\hat{\stateVect}}}
\newcommand{\inpDiag}{\hat{\inp}} %input to the diagonal block 
\newcommand{\inputCoef}{g}
\newcommand{\inpVect}{{u}}
\newcommand{\outVect}{{\pos}}
\newcommand{\outVectMod}{\tilde{\outVect}}
\newcommand{\stateVectDer}{\dot{\stateVect}}
\newcommand{\stateVectModDer}{\dot{\stateVectMod}}

%overall formation matrices
\newcommand{\matA}{{A}}
\newcommand{\matB}{{B}}
\newcommand{\matC}{{C}}
\newcommand{\matD}{{D}}
%small open loop matrices
\newcommand{\matAi}{{A}}
\newcommand{\matBi}{{B}}
\newcommand{\matCi}{{C}}
\newcommand{\matDi}{{D}}
\newcommand{\matAiMod}{\bar{\matAi}}
\newcommand{\matAMod}{\bar{\matA}}
\newcommand{\matBMod}{\bar{\matB}}
%identity matrices and vectors
\newcommand{\Id}{{I}}
\newcommand{\In}{\Id_\olOrd}
\newcommand{\IN}{\Id_\numVeh}
\newcommand{\Ino}{\Id_{\vehNumOut}}
\newcommand{\oneVect}{\mathbf{1}}
\newcommand{\canonVect}{e}

%% ------------- transfer functions --------------
\newcommand{\diagTransBlock}{{F}}
\newcommand{\diagTransBlockWn}{\diagTransBlock_{\wn}}
\newcommand{\diagTransBlockEig}{T}
\newcommand{\diagTransBlockEigZ}{Z}
\newcommand{\diagTransBlockEigZij}{Z_{ij}}
\newcommand{\diagTransBlockEigWn}{\diagTransBlockEig_{\spatEig_j}}
\newcommand{\diagTransBlockMin}{\diagTransBlock_{\min}}
\newcommand{\diagTransBlockMax}{\diagTransBlock_{\max}}
\newcommand{\diagTransBlockEigMin}{\diagTransBlockEig_{\spatEig_{\min}}}
\newcommand{\diagTransBlockEigMax}{\diagTransBlockEig_{\spatEig_{\max}}}
\newcommand{\diagTransBlockN}{\diagTransBlockEig_{\numVeh}}
\newcommand{\diagTransBlockCO}{\diagTransBlockEig_{CO}}
\newcommand{\matJTrans}{\mathbf{\matJ}_\diagTransBlock}
\newcommand{\setZi}{\mathcal{J}}
%% -------------- Trnasfer function from C to O -----------------
\newcommand{\tranFunCo}{T_{co}}
\newcommand{\lengthShortPath}{l}
%%--------------- Single integrator dynamics transfer functions --------------%%
\newcommand{\singleIntNumPol}{Q}
\newcommand{\singleIntDenPol}{P}

%% Norms
\newcommand{\hinfnorm}{\mathcal{H}_{\infty}}

%% coefficients
\newcommand{\eigVectGenCoef}{\alpha}


% % Subscripts

% Derivatives of one car
% general words
\newcommand{\pde}{PDdE}

% General symbols
\newcommand{\dd}{\mathrm{d}}

==> version 2/inputlatex.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%To draw commutative diagrams.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amscd}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}

%\input{pepet.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Valencian Definitions
%Uso de las definiciones valencianas%
%Theorem
%\begin{theo}\label{***}Statement of theorem \end{theo}
%\begin{prop}\label{***}Statement of theorem \end{prop}
%\begin{lem}\label{***}Statement of theorem \end{lem}
%\begin{cory}\label{***}Statement of theorem \end{cory}
%\begin{rem}\label{***}Statement of theorem \end{rem}
%when needed:
%\setcounter{figure}{0}
%\setcounter{equation}{0}
%\setcounter{theorem}{0}
%\begin{proof}  Proof \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand{\theequation}{\thesection.\arabic{equation}}
%\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\newtheorem {theo} {\bf Theorem}
\newtheorem {prop} [theo] {\bf Proposition}
\newtheorem {cory} [theo] {\bf Corollary}
\newtheorem {lem} [theo] {\bf Lemma}
\newtheorem {defn} [theo] {\bf Definition}
\newtheorem {conj} [theo] {\bf Conjecture}
\newtheorem {exam} [theo] {\bf Example}
\newtheorem {rem} [theo] {\bf Remark}
\newtheorem {claim} [theo] {\bf Claim}
\newtheorem {assum} {\bf Assumption}
\newcommand{\QED}{\hfill \CaixaPreta \vspace{6mm}}
\def\CaixaPreta{\vrule Depth0pt height6pt width6pt}
\newenvironment{remark}{\begin{rem}\begin{rm}}{\end{rm}
\nopagebreak\hfill$\Box$\end{rem}\par\vspace{\partopsep}}
\newenvironment{defin}{\begin{DEFCURSIVA}\begin{rm}}{\end{rm}\end{DEFCURSIVA}}
\newenvironment{proclama}[1]{\par\vspace{\topsep}\noindent{\bf #1}
\begin{em}}{\end{em}\par\vspace{\topsep}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dpy}{\displaystyle}
%eqn array with numbered lines:
%use & to align, \\ for new line, \\[0.4cm] for new line and add'l vert. space.
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
%eqn array no number:
\newcommand{\benn}{\begin{eqnarray*}}
\newcommand{\eenn}{\end{eqnarray*}}
%single eqn numbered:
\newcommand{\bse}{\begin{equation}}
\newcommand{\ese}{\end{equation}}
%single eqn no number:
\newcommand{\bsenn}{\begin{displaymath}}
\newcommand{\esenn}{\end{displaymath}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Some Functions (math style)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\logand}{\;\;{\rm and }\;\;}
\newcommand{\for}{\;\;{\rm for }\;\;}
\newcommand{\logor}{\;\;{\rm or }\;\;}
\newcommand{\logif}{\;\;{\rm if }\;\;}
\newcommand{\logelse}{\;\;{\rm else }\;\;}
\newcommand{\then}{\;\;{\rm then }\;\;}
\newcommand{\where}{\;\;{\rm where }\;\;}
\newcommand{\with}{\;\;{\rm with }\;\;}
\newcommand{\such}{\;\;{\rm such\; that }\;\;}
\newcommand{\limcap}{\;{\rm d }\,}
\newcommand{\Tr}{\;{\rm Tr }\,}
\newcommand{\Hd}{\;{\rm Hd }\,}
\newcommand{\atanh}{\;{\rm arctanh }\,}
\newcommand{\Hdim}{\;{\rm Hdim }\,}
\newcommand{\Hlim}{\;{\rm Hlim }\,}
\newcommand{\card}{\;{\rm card }\,}
\newcommand{\Id}{\,{\rm Id}\,}
%\newcommand{\mod}{\bmod}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Other
%%('re' is added because \O and \S are existing commands)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\O}{\mathbb{O}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\C}{\mbox{I${\!\!\!}$C}}
%\renewcommand{\O}{\mbox{I${\!\!\!}$O}}
%\renewcommand{\H}{\mbox{I${\!\!\!}$H}}
%\newcommand{\Q}{\mbox{I${\!\!\!}$Q}}
%\newcommand{\G}{\mbox{I${\!\!\!}$G}}
%\newcommand{\T}{\mbox{T${\!\!\!}$T}}
%\newcommand{\N}{\mbox{I${\!}$N}}
%\newcommand{\R}{\mbox{I${\!}$R}}
%\newcommand{\D}{\mbox{I${\!}$D}}
%\newcommand{\Z}{\mbox{Z${\!\!}$Z}}
%\renewcommand{\S}{\mbox{S${\!\!\!\!}$S}}
\newcommand{\CaixaBranca}{$\Box$}
\newcommand{\creu}{{\rule[-0.1mm]{2mm}{0.2mm}\rule{0.1mm}{2.5mm}}}
\newcommand{\ca}{\c ca }
\newcommand{\co}{\c co }
\newcommand{\mv}{mente, }
\newcommand{\caop}{\c c\~ao. }
\newcommand{\caov}{\c c\~ao, }
\newcommand{\coesp}{\c c\~oes. }
\newcommand{\coesv}{\c c\~oes, }
\newcommand{\cao}{\c c\~ao }
\newcommand{\CAO}{\c C\~AO }
\newcommand{\coes}{\c c\~oes }
\newcommand{\COES}{\c C\~OES }
\newcommand{\sao}{s\~ao }
\newcommand{\SAO}{S\~AO }
\newcommand{\m}{mente }
\newcommand{\ii}{\'{\i}}

%% Constants
\newcommand{\numVeh}{N}

%% Notation of variables
\newcommand{\subvel}{v}		%subscript for velocity
\newcommand{\subpos}{x}		%subscript for position
\newcommand{\fric}{a} 		%friction
\newcommand{\pos}{z}  		%position in error dynamics
\newcommand{\posdist}{x}	%position with distance to the leader
\newcommand{\vel}{v}		%velocity
\newcommand{\contState}{c}	%controller state
\newcommand{\inp}{u}		%input to the vehicle
\newcommand{\regerr}{\epsilon}		%regulation error
\newcommand{\gv}{g_v}		%gain of velocity error
\newcommand{\gx}{g_x}		%gain of position error
\newcommand{\asym}{\rho}
\newcommand{\rx}{\asym_\subpos}	%asymmetry in position
\newcommand{\rv}{\asym_\subvel}	%asymmetry in velocity
\newcommand{\bx}{\beta_\subpos}			%beta_x = 2 \asymPos+1
\newcommand{\bv}{\beta_\subvel}			%beta_v = 2 \asymVel+1
\newcommand{\state}{x}		%state vector

%Signal properties
\newcommand{\wv}{c}		%wave velocity general
\newcommand{\cp}{c_+}	%wave velocity towards the end
\newcommand{\cm}{c_-}	%wave velocity towards the leader
\newcommand{\ampl}{A}	%amplitude of the oscillations
\newcommand{\period}{T}	%period of the oscillation
\newcommand{\erl}{e}	%spacing error to the leader
\newcommand{\areaosc}{E}	%area of the error of the agent to the leader

%% Notation of transfer functions
\newcommand{\vehTf}{G} 		%transfer function of the vehicle
\newcommand{\contTf}{C}		%transfer function of the general controller
\newcommand{\contFront}{\contTf_f}	%transfer function of the front controller
\newcommand{\contRear}{\contTf_r}	%transfer function of the rear controller

%%Matrices
\newcommand{\lapl}{L}		%Laplacian in general
\newcommand{\lv}{\lapl_\subvel} 	%Laplacian for velocity path graph
\newcommand{\lx}{\lapl_\subpos}		%Laplacian for position path graph
\newcommand{\laplc}{\hat{\lapl}}

\newcommand{\lvc}{\laplc_\subvel} 	%Laplacian for velocity circular graph
\newcommand{\lxc}{\laplc_\subpos}		%Laplacian for position circular graph
\newcommand{\systMat}{M_\numVeh}	%overall system matrix in state space
\newcommand{\systMatCirc}{\hat{M}_\numVeh} %overall system matrix for circular
% system
\newcommand{\eigVectM}{u}			%eigenvector of state matrix \systMat

\newcommand{\eigVectL}{w}			%eigenvector of Laplacian
\newcommand{\sfr}{\phi}		%frequency of the eigenvector of the Laplacian
\newcommand{\eigl}{\lambda}			%eigenvalue of the Laplacian
\newcommand{\eiglx}{\eigl_\subpos}	%eigenvalue of Laplacian for position
\newcommand{\eiglv}{\eigl_\subvel}	%eigenvalue of Laplacian for velocity
\newcommand{\eigm}{\nu}				%eigenvalue of the overall system matrix \systMat 
\newcommand{\eigmcoef}{n}		%coefficient in taylor series expansion of \eigm
\newcommand{\charpol}{p}			%characterisic polynomial of one diagonal system
\newcommand{\charpolreal}{\hat{\charpol}}	%polymomial with only real
% coefficients




==> version 2/notation.tex <==
%% Notation commands
\newcommand{\pos}{y} %car's position 
\newcommand{\err}{\tilde{e}} %spacing error 
\newcommand{\inp}{r} %input of the car -acceleration
\newcommand{\totalInput}{u}
\newcommand{\relCoupling}{c}

\newcommand{\dreference}{d_{\mathrm{ref}}} %reference distance
\newcommand{\drefVect}{{d}}
\newcommand{\vel}{v}
\newcommand{\weightGain}{\mu}

%% ODE coefficients
\newcommand{\contNumCoef}{q}
\newcommand{\contDenCoef}{p}
\newcommand{\vehNumCoef}{b}
\newcommand{\vehDenCoef}{a}
\newcommand{\olnum}{\psi} %numarator of open loop
\newcommand{\olden}{\phi} %denominator of open loop


%% Transfer functions
\newcommand{\vehicleTf}{G}
\newcommand{\controllerTf}{R}
\newcommand{\systemOutput}{y}
\newcommand{\systemOutputVect}{{\systemOutput}}
\newcommand{\controlEffort}{u}
\newcommand{\controlEffortVect}{{\controlEffort}}
\newcommand{\relOutDif}{\tilde{\systemOutput}}
\newcommand{\relOutDifVect}{\mathbf{\relOutDif}}
\newcommand{\regError}{E}
\newcommand{\regErrorVect}{\mathbf{\regError}}
\newcommand{\openLoop}{M}
\newcommand{\openLoopGain}{\openLoop_{\min}}
\newcommand{\olNumMat}{N}
\newcommand{\outWeightMat}{W}

\newcommand{\contNumOrd}{w}
\newcommand{\contDenOrd}{v}
\newcommand{\vehNumOrd}{m}
\newcommand{\olOrd}{n}
\newcommand{\wn}{i}

%weights of asymmetric bidirectional control
\newcommand{\wf}{1}
\newcommand{\wb}{\epsilon}
\newcommand{\wbmax}{\wb_{\max}}


% Constants
\newcommand{\numVeh}{N}

% % Functions
\newcommand{\drefWn}{\dreference_\wn}

% assumption

%%% ------- matrices and vectors -----------------
% laplacian and its eigenpairs
\newcommand{\lapl}{{L}}
\newcommand{\lapllf}{\lapl_{lf}} % laplacian with two leaders
\newcommand{\lapll}{\lapl_l} %laplacian with one leader
\newcommand{\redLapl}{{\lapl_\mathrm{r}}}
\newcommand{\redLaplCO}{\hat{\lapl}}
\newcommand{\redLapllf}{\bar{\lapl}_{lf}}
\newcommand{\laplz}{\lapl_z} % Laplacian to obtain zeros of the system
\newcommand{\spatEig}{\lambda} %laplacian eigenvalues
\newcommand{\spatEigWn}{\lambda_\wn}
\newcommand{\spatEigMin}{\spatEig_{\min}}
\newcommand{\spatEigMax}{\spatEig_{\max}}
\newcommand{\eigVect}{v} %laplacian eigenvectors
\newcommand{\eigVectGen}{\bar{\eigVect}}
\newcommand{\eigVectWn}{\eigVect_{\wn}}
\newcommand{\spatFreqWn}{\theta_\wn} %spatial frequency
\newcommand{\charPolCoef}{\alpha}
%zeros
\newcommand{\spatEigZ}{\gamma}
%jordan form
\newcommand{\matJ}{{J}}
\newcommand{\matEigVect}{{V}}
%graph 
\newcommand{\graph}{\mathcal{G}}
\newcommand{\vertSet}{\mathcal{V}}
\newcommand{\edgeSet}{\mathcal{E}}
\newcommand{\contNode}{C}
\newcommand{\obsvNode}{O}
\newcommand{\distance}{d}
\newcommand{\distanceCO}{\distance_{CO}}
\newcommand{\weight}{w}
\newcommand{\weightCO}{\weight_{CO}}

%state vector and matrices
\newcommand{\stateVect}{{x}}
\newcommand{\stateVectMod}{{\hat{\stateVect}}}
\newcommand{\inpDiag}{\hat{\inp}} %input to the diagonal block 
\newcommand{\inputCoef}{g}
\newcommand{\inpVect}{{u}}
\newcommand{\outVect}{{\pos}}
\newcommand{\outVectMod}{\tilde{\outVect}}
\newcommand{\stateVectDer}{\dot{\stateVect}}
\newcommand{\stateVectModDer}{\dot{\stateVectMod}}

%overall formation matrices
\newcommand{\matA}{{A}}
\newcommand{\matB}{{B}}
\newcommand{\matC}{{C}}
\newcommand{\matD}{{D}}
%small open loop matrices
\newcommand{\matAi}{{A}}
\newcommand{\matBi}{{B}}
\newcommand{\matCi}{{C}}
\newcommand{\matDi}{{D}}
\newcommand{\matAiMod}{\bar{\matAi}}
\newcommand{\matAMod}{\bar{\matA}}
\newcommand{\matBMod}{\bar{\matB}}
%identity matrices and vectors
\newcommand{\Id}{{I}}
\newcommand{\In}{\Id_\olOrd}
\newcommand{\IN}{\Id_\numVeh}
\newcommand{\Ino}{\Id_{\vehNumOut}}
\newcommand{\oneVect}{\mathbf{1}}
\newcommand{\canonVect}{e}

%% ------------- transfer functions --------------
\newcommand{\diagTransBlock}{{F}}
\newcommand{\diagTransBlockWn}{\diagTransBlock_{\wn}}
\newcommand{\diagTransBlockEig}{T}
\newcommand{\diagTransBlockEigZ}{Z}
\newcommand{\diagTransBlockEigZij}{Z_{ij}}
\newcommand{\diagTransBlockEigWn}{\diagTransBlockEig_{\spatEig_j}}
\newcommand{\diagTransBlockMin}{\diagTransBlock_{\min}}
\newcommand{\diagTransBlockMax}{\diagTransBlock_{\max}}
\newcommand{\diagTransBlockEigMin}{\diagTransBlockEig_{\spatEig_{\min}}}
\newcommand{\diagTransBlockEigMax}{\diagTransBlockEig_{\spatEig_{\max}}}
\newcommand{\diagTransBlockN}{\diagTransBlockEig_{\numVeh}}
\newcommand{\diagTransBlockCO}{\diagTransBlockEig_{CO}}
\newcommand{\matJTrans}{\mathbf{\matJ}_\diagTransBlock}
\newcommand{\setZi}{\mathcal{J}}
%% -------------- Trnasfer function from C to O -----------------
\newcommand{\tranFunCo}{T_{co}}
\newcommand{\lengthShortPath}{l}
%%--------------- Single integrator dynamics transfer functions --------------%%
\newcommand{\singleIntNumPol}{Q}
\newcommand{\singleIntDenPol}{P}

%% Norms
\newcommand{\hinfnorm}{\mathcal{H}_{\infty}}

%% coefficients
\newcommand{\eigVectGenCoef}{\alpha}


% % Subscripts

% Derivatives of one car
% general words
\newcommand{\pde}{PDdE}

% General symbols
\newcommand{\dd}{\mathrm{d}}
